The Consensus Number of a Cryptocurrency (Extended Version)

Many blockchain-based algorithms, such as Bitcoin, implement a decentralized asset transfer system, often referred to as a cryptocurrency. As stated in the original paper by Nakamoto, at the heart of these systems lies the problem of preventing double-spending; this is usually solved by achieving consensus on the order of transfers among the participants. In this paper, we treat the asset transfer problem as a concurrent object and determine its consensus number, showing that consensus is, in fact, not necessary to prevent double-spending. We first consider the problem as defined by Nakamoto, where only a single process---the account owner---can withdraw from each account. Safety and liveness need to be ensured for correct account owners, whereas misbehaving account owners might be unable to perform transfers. We show that the consensus number of an asset transfer object is $1$. We then consider a more general $k$-shared asset transfer object where up to $k$ processes can atomically withdraw from the same account, and show that this object has consensus number $k$. We establish our results in the context of shared memory with benign faults, allowing us to properly understand the level of difficulty of the asset transfer problem. We also translate these results in the message passing setting with Byzantine players, a model that is more relevant in practice. In this model, we describe an asynchronous Byzantine fault-tolerant asset transfer implementation that is both simpler and more efficient than state-of-the-art consensus-based solutions. Our results are applicable to both the permissioned (private) and permissionless (public) setting, as normally their differentiation is hidden by the abstractions on top of which our algorithms are based.

==> introduction.tex <==
\section{Introduction}
\label{sec:intro}

The Bitcoin protocol, introduced in 2008 by Satoshi Nakamoto,  implements a \emph{cryptocurrency}: an electronic decentralized asset transfer system~\cite{nakamotobitcoin}.
% without any central authority.
Since then, many alternatives to Bitcoin came to prominence.
These include major cryptocurrencies such as Ethereum~\cite{ethereum} or Ripple~\cite{rapoport2014ripple}, as well as systems sparked from research or industry efforts such as Bitcoin-NG~\cite{eyal16bitcoinng}, Algorand~\cite{gilad2017algorand}, ByzCoin~\cite{kogi16byzcoin}, Stellar~\cite{mazieres2015stellar}, Hyperledger~\cite{hyperledger}, Corda~\cite{he16corda}, or Solida~\cite{abr16solida}.
Each alternative brings novel approaches to implementing decentralized transfers, and sometimes offers a more general interface (known as smart contracts~\cite{sz97smartcontr}) than the original protocol proposed by Nakamoto.
They improve over Bitcoin in various aspects, such as performance, energy-efficiency, or security.

A common theme in these protocols, whether they are for basic transfers~\cite{kok18omniledger} or smart contracts~\cite{ethereum},
is that they seek to implement a \emph{blockchain}---a distributed ledger where all the transfers in the system are totally ordered.
Achieving total order among multiple inputs (e.g., transfers) is fundamentally a hard task, equivalent to solving \emph{consensus}~\cite{Her91,HT93}.
Consensus~\cite{FLP85}, a central problem in distributed computing, is known for its notorious difficulty.
It has no deterministic solution in asynchronous systems
if just a single participant can fail~\cite{FLP85}.
Partially synchronous consensus algorithms are tricky to implement correctly~\cite{abrah17revisiting,cac17blwild,clement09making}
and face tough trade-offs between performance, security, and energy-efficiency~\cite{antoni18smr,ber89optimal,gue18blockchain,vuko15quest}.
Not surprisingly, the consensus module is a major bottleneck in blockchain-based protocols~\cite{he16corda,sou18byzantine,vuko15quest}.
% Numerous solutions have emerged to alleviate this problem~\cite{gol18sbft,he16corda}. Typical techniques seek to employ a form of sharding~\cite{kok18omniledger}, for instance, or to use a committee-based optimization~\cite{eyal16bitcoinng,gilad2017algorand}.
%% With \name, we circumvent this main bottleneck, yielding new solutions that bypass consensus altogether.

A close look at Nakamoto's original paper reveals that the central issue in implementing 
a decentralized asset transfer system (i.e., a cryptocurrency)
is preventing \emph{double-spending}, i.e., spending the same money more than once~\cite{nakamotobitcoin}.
%This is known as \emph{double-spending}.
Bitcoin and numerous follow-up systems typically assume that total order---and thus consensus---is vital to preventing double-spending~\cite{gar15backbone}.
There seems to be a common belief, indeed, that a consensus algorithm is essential for implementing decentralized asset transfers~\cite{BonneauMCNKF15,gue18blockchain,kar18vegvisir,nakamotobitcoin}.

As our main result in this paper, we show that this belief is false.
We do so by casting the asset transfer problem as a \emph{sequential object type} and determining that it has \emph{consensus number} $1$ in Herlihy's hierarchy \cite{Her91}.%
\footnote{The consensus number of an object type is the maximal number of processes that can solve consensus using only read-write shared memory and arbitrarily many objects of this type.}

%% Our first contribution is a precise definition of asset transfer as a sequential object type that we call \textsf{asset-transfer}. We then determine its  \emph{consensus number} in the sense of \cite{Her91}.
% We start from this model as it allows us to study the relation between the transfer object and consensus, and later present our result in the message passing model with Byzantine failures.
% We first show that an \textsf{asset-transfer} object has consensus number \emph{one} by implementing it in the read-write shared memory model. In other words, decentralized asset transfer does not need consensus in its implementation, and we can avoid maintaining a total order among transfers.
% To get an intuition why total order is not necessary, consider a set of users
% who transfer money between their accounts in a decentralized manner.
% For simplicity, assume the full replication model, where every user maintains a copy of the state of every account.
% We observe that most operations in a transfer system \emph{commute}, i.e., different users can apply the operations in arbitrary order, resulting in the same final state.
% For instance, a transfer $T_1$ from Alice to Bob commutes with a transfer $T_2$ from Carol to Drake.
% This is because the two transfers involve different accounts.
% In the absence of other transfers, $T_1$ and $T_2$ can be applied in different orders by different users, without affecting correctness.
% Consider now a more interesting case when two transfers involve the same account.
% For example, let us throw into the mix a transfer $T_0$ from Alice to Carol.
% Assume that Alice issues $T_0$ before she issues $T_1$.
% Note that $T_0$ and $T_1$ do not commute, because they involve the same account---that of Alice---and
% it is possible that she cannot fulfill both $T_0$ and $T_1$ (due to insufficient balance).
% We say that $T_1$ depends on $T_0$, and so $T_0$ should be applied before $T_1$.
% Furthermore, suppose that Carol does not have enough money in her account to fulfill $T_2$ before she receives transfer $T_0$ from Alice.
% In this case, transfer $T_2$ depends on $T_0$.
% Thus, all users should apply $T_0$ before applying $T_2$, while transfers $T_1$ and $T_2$ still commute.
% The partial ordering among these three transfers is in fact given by a \emph{causality} relationship.
% In~\Cref{fig:scenario-intro} we show the scenario with these three transfers and the causality relation between them.
% Intuitively, the general ordering constraint we seek to enforce is that every outgoing transfer for an account causally depends on all preceding transfers involving that---and only that---account.
% \begin{figure}[h!]
% \includegraphics[width=0.4\columnwidth]{./figs/scenario-intro}
% \caption{A simple scenario illustrating, on the left side, three transfers among four participants.
% On the right side, we depict the dependencies among these three transfers.
% The dependencies are established by a causality-based ordering relationship.}
% \label{fig:scenario-intro}
% \end{figure}

The intuition behind this result is the following.
An asset transfer object maintains a set of accounts.
%and where processes are allowed to transfer assets between accounts.
Each account is associated with an \emph{owner} process that is the only one allowed to issue transfers withdrawing from this account.
Every process can however read the balance of any account.

The main insight here is that relating accounts to unique owners obviates the need for consensus.
It is the owner that decides on the order of transfers from its own account, without the need to agree with any other process---thus the consensus number 1.
Other processes only validate the owner's decisions, ensuring that causal relations across accounts are respected.
% [[PK not applicable to the benign failure case 
% If an account owner proposes two conflicting transfers, the processes may never reach consensus on which of them to consider valid and which to reject, and may simply ignore both.
We describe a simple asset transfer implementation using  atomic-snapshot memory~\cite{AADGMS93}.
%In our asset transfer implementation, the performed transfer operations are shared using atomic-snapshot memory~\cite{AADGMS93}.
%
A withdrawal from an account is validated by relating the withdrawn amount with the incoming transfers found in the memory snapshot.
%
Intuitively, as at most one withdrawal can be active on a given account at a time, it is safe to declare the validated operation as successful and post it in the snapshot memory.                
%Our implementation of \textsf{asset-transfer} is based on an atomic snapshot object that is known to have a wait-free implementation in read-write shared memory~\cite{AADGMS93}.
%Such an object consists of entries, each of which is assigned to a single process that can write to it.
%Moreover, any process can atomically read the content of all entries.
%We use the atomic snapshot object to represent the state of the accounts in our asset transfer system.
%One entry of the atomic snapshot object corresponds to one account, the process assigned to the entry being the account owner.
%]]

We also present a natural generalization of our result to the setting in which multiple processes are allowed to withdraw from the same account.
A \emph{$k$-shared} asset-transfer object allows up to $k$ processes to execute outgoing transfers from the same account.
We prove that such an object has consensus number $k$ and thus allows for implementing \emph{state machine replication} (now often referred to as \emph{smart contracts}) among the $k$ involved processes using $k$-consensus objects~\cite{JT92}.
% Our proof shows that both the upper bound and the lower bound on the consensus number of $k$-shared \textsf{asset-transfer} is $k$.
%
%[[PK 
\ignore{
We prove the lower bound by providing a wait-free implementation of consensus in a shared memory system with $k$ processes equipped with a $k$-shared asset transfer object.
Each process first announces its proposed value in a dedicated (per-process) register,
and then tries to perform a transfer from a shared account.
We choose the initial account balance and the withdrawn amounts so that (1)~exactly one withdrawal wins and (2)~the remaining balance identifies the winner process.
%
The upper bound proof makes use of a $k$-consensus object~\cite{JT92} (known to have consensus number $k$).
}
% ]]
%[[PK shorten, the tools are standard
We show that $k$-shared asset transfer has consensus number
% at most
$k$ by reducing it to $k$-consensus (known to have consensus number $k$) and reducing $k$-consensus to asset transfer.
%Our reduction borrows concepts from universal construction of sequential objects on top of consensus:
%the $k$ owners of an account use a sequence of $k$-consensus objects to agree on the order of outgoing transfers and their results.
%We then show that $k$-shared asset transfer has consensus number at least $k$ by devising an algorithm where up to $k$ processes solve consensus by transferring distinct amounts from the same $k$-shared account in an asset transfer object.   
%]]
%
% We store the state of the accounts in an atomic snapshot object as described above.

Having established the relative ease of the asset transfer problem using the shared memory model,
we also present a practical solution to this problem in the %more realistic
setting of Byzantine fault-prone processes communicating via message passing.
This setting matches realistic deployments of distributed systems.
We describe an asset transfer implementation that does not resort to consensus.
Instead, the implementation relies on a \emph{secure broadcast} primitive that ensures uniform reliable delivery with only weak ordering guarantees~\cite{ma97secure,MR97srm}, circumventing hurdles imposed by consensus.
% This allows our solution to be simpler, more efficient, and fully asynchronous.
% \cmt{PK}{Somethiong about efficiency here?}
%
In the $k$-shared case, our results imply that to execute some form of \emph{smart contract} involving $k$ users,
consensus is only needed among these $k$ nodes and not among all nodes in the system.
In particular, should these $k$ nodes be faulty, the rest of the accounts will not be affected.

% \cmt{ADI}{Move this paragraph before the previous one, and shorten the previous one.}
To summarize, we argue that treating
%[[PK more to the point?
the asset transfer problem as a concurrent data structure
%\emph{double-spending} as
%a distributed computing problem
and measuring its hardness through the lense of distributed computing help understand
it and devise better solutions to it.
% We prove our results in the simpler shared memory model with benign failures and then discuss how they translate to message passing with Byzantine failures.
%]]

% \cmt{MP}{Extend this in case we decide to have an appendix with the message passing algorithm.}
% Secure broadcast is an abstraction that, in short, ensures uniform reliable message delivery in FIFO order despite a Byzantine environment, if the message sender is correct.
% It has been well studied \cite{br85acb} and is strictly weaker than consensus.

%% Whether for the deterministic or probabilistic model, our \namemp\ algorithms are both simpler and faster than solutions based on consensus.
%% In systems of up to $100$ replicas, regardless of system size, \namedet\ outperforms consensus-base
%% d solutions offering a throughput improvement ranging from $1.5x$ to $6x$, while achieving a decrease in latency of up to $2x$.
%% \nameprob\ obtains \emph{sub-second} transfer execution on a global scale deployment of thousands o
%% f nodes.
%% \cmt{RG}{I believe it is crucial to talk about number of lines of code (order of magnitude less) and say that this is crucial for proving and testing the system. 
%% You might also say that our protocols are all built on solid foundations and proven correct}
%% \cmt{YAP}{not shown in this version... it would be great to mention the complexity instead!}


The rest of this paper is organized as follows.
We first give the formal definition of the shared memory model and the asset transfer object type~(\cref{sec:model}).
Then, we show that this object type has consensus number $1$~(\cref{sec:avoiding-consensus}).
Next, we generalize our result by proving that a $k$-shared asset transfer object has consensus number $k$ (\cref{sec:k-consensus}).
Finally, we describe the implications of our results in the message passing model with Byzantine faults (\cref{sec:msg-passing-implications,sec:generalize-shared}) and discuss related work (\cref{sec:related-work}).
% For space limitations, we defer the precise description of the Byzantine message passing model, the corresponding asset transfer algorithm with correctness proof, and a discussion on how to generalize it to the $k$-shared case, to appendices \ref{sec:def-byz}, \ref{sec:at-in-msg-passing} and \ref{sec:generalize-shared}, respectively.
% Appendix \ref{sec:message-passing}.


==> sections/conclusions.tex <==
%!TEX root = ../main.tex

\section{Concluding Remarks}
\label{sec:conclusions}

We established our main results in a shared memory system with crash failures, proving that consensus is not necessary for implementing an asset transfer system, i.e., a cryptocurrency.
Moreover, a natural generalization of such a system where up to $k$ processes have access to atomic operations on the same account has consensus number $k$.

Our result extends to the message passing system with Byzantine failures.
In a straightforward way, one can emulate shared read-write memory in a Byzantine message passing system with less than one third of faulty processes \cite{imbs16byzshm}
and implement an asset transfer on top of this abstraction.\cmt{MP}{Complexity}
However, we can implement asset transfer in a message passing system more efficiently,
directly using a secure broadcast abstraction that provides uniform reliable delivery with weak (weaker than FIFO) ordering guarantees.
Such an implementation still does not rely on agreement, is simpler, and remains fully asynchronous.
For the exact algorithm and its correctness proof, we refer the interested reader to the appendix,
where we also explain how our algorithm generalizes to the $k$-shared case.

We also considered a fixed set of $n$ processes and did not address a dynamic setting, involving the addition or removal of processes.
We believe that our results could also be ported to a dynamic setting in a consensusless manner,
following the path of Aguilera et al. \cite{agu10reconfig, agu11das}, showing how to emulate a shared memory in a dynamic message passing system without consensus.
We conjecture that their "dynamic emulation" can also be applied to a setting with Byzantine failures.

In order to deploy an account transfer system in a large-scale, public (permissionless) setting, two crucial problems need to be adressed: scalability and resistance to Sybil attacks.
Both these issues can be addressed through randomization.
While in this paper we focused on deterministic solutions based on a secure broadast primitive with well known implementations,
in a companion paper, we present a highly scalable randomized secure broadcast implementation [hidden reference].
To ensure Sybil resistance, various approaches, including the infamouse proof-of-work scheme, can be employed.
Yet, these do not need to be as expensive as in blockchain, where the goal of proof-of-work is both to prevent Sybil attacks and to elect a unique consensus leader:
the latter is precisely what makes the scheme so expensive.

\ignore{
In this paper we revisited the problem of implementing an asset transfer system.
Since the rise of the Bitcoin cryptocurrency, this problem has garnered significant innovation.
Most of the innovation, however, has focused on improving the original solution which Bitcoin proposed, namely, that of using a consensus mechanism to build a blockchain where transactions across the whole system are totally ordered.

% We did not aim to investigate current consensus-based solutions and push the envelope on performance or other metrics.
We showed that we can implement an asset transfer system (i.e., a cryptocurrency) without resorting to consensus.
To this end, we first precisely defined the \textsf{asset-transfer} object type and proved that it has consensus number \emph{one} if a single account is not shared by multiple processes.
That is, it occupies the lowest rank of the consensus hierarchy and can be implemented without the need for solving consensus.

A consensusless solution for decentralized transfers has multiple advantages.
In particular, this means that cryptocurrencies are not subject to the FLP impossibility~\cite{FLP85}.
% Additionally,  is significantly simpler than consensus-based solutions (because it relies on a simpler secure broadcast primitive).

We also extended our result to more general \textsf{asset-transfer} objects, where accounts may be shared by up to $k$ processes.
We proved that such a $k$-owned \textsf{asset-transfer} is equivalent to $k$-consensus and thus has consensus number $k$.
% We proved this surprising result by borrowing from the theory of concurrent objects, and then leveraged the result to build \name, the first consensusless transfer system.
}

